Quantum (sl_n, \land V_n) link invariant and matrix factorizations

M. Khovanov and L. Rozansky gave a categorification of the HOMFLY-PT polynomial. This study is a generalization of the Khovanov-Rozansky homology. We define a homology associated to the quantum $(sl_n,\land V_n)$ link invariant, where $\land V_n$ is the set of the fundamental representations of the quantum group of $sl_n$. In the case of a [1,k]-colored link diagram, we prove that its homology is a link invariant. In the case of an [i,j]-colored link diagram, we define a normalized Poincare polynomial of its homology and prove the polynomial is a link invariant.

==> figure/r1c.tex <==
%WinTpicVersion3.08
\unitlength 0.1in
\begin{picture}(3.500,3.00)(0.500,-4.200)
% VECTOR 2 0 3 0
% 2 300 1000 300 200
% 
\special{pn 8}%
\special{pa 200 600}%
\special{pa 200 200}%
\special{fp}%
\end{picture}%


==> figure/r2c.tex <==
\unitlength 0.1in
\begin{picture}(4.500,3.00)(1.7500,-4.200)
\special{pn 8}%
\special{pa 200 600}%
\special{pa 200 200}%
\special{fp}%
% VECTOR 2 0 3 0
% 2 600 1000 600 600
% 
\special{pn 8}%
\special{pa 600 600}%
\special{pa 600 200}%
\special{fp}%
\end{picture}%

